Meta-Learning MCMC Proposals

Effective implementations of sampling-based probabilistic inference often require manually constructed, model-specific proposals. Inspired by recent progresses in meta-learning for training learning agents that can generalize to unseen environments, we propose a meta-learning approach to building effective and generalizable MCMC proposals. We parametrize the proposal as a neural network to provide fast approximations to block Gibbs conditionals. The learned neural proposals generalize to occurrences of common structural motifs across different models, allowing for the construction of a library of learned inference primitives that can accelerate inference on unseen models with no model-specific training required. We explore several applications including open-universe Gaussian mixture models, in which our learned proposals outperform a hand-tuned sampler, and a real-world named entity recognition task, in which our sampler yields higher final F1 scores than classical single-site Gibbs sampling.

==> 40train.tex <==
%auto-ignore
%!TEX root = paper.tex

Suppose a way to draw sample pairs $(\mathbf{x}, \psi)$. In practice, this can be from using a prior on $\psi$, from a training data set, etc.

Let $(\mathbf{x}^{(i)}, \psi^{(i)})$ be samples. Objective is to minimize loss:

\resizebox{\columnwidth}{!}{
 \begin{minipage}{\linewidth}
    \begin{align}
        L & = \mathbb{E}_{\mathbf{x}, \psi}[\kl{\Pr[\mathbf{X}_S|\mathbf{x}_{G - S}; G, \psi]}{\NN_{G, \theta}(\mathbf{X}_S|\mathbf{x}_{\text{N}(S;G)}, \psi_{\text{N}(S;G)})}] \nonumber \\
        % & \approx \frac{1}{n} \sum_{i = 1}^n \kl{\Pr[\mathbf{X}_S|\mathbf{x}^{(i)}_{\text{N}(S;G)}; G, \psi^{(i)}]}{\NN_{G, \theta}(\mathbf{X}_S|\mathbf{x}^{(i)}_{\text{N}(S;G)}, \psi^{(i)})} \nonumber \\
        & \approx - \frac{1}{n} \sum_{i = 1}^n \log \NN_{G, \theta}(\mathbf{x}^{(i)}_S|\mathbf{x}^{(i)}_{\text{N}(S;G)}, \psi^{(i)}_{\text{N}(S;G)}) + C
    \end{align}
\end{minipage}
}

Mini-batch SGD.

\reminder{do we need to discuss special case or practical issue?}

